Automated CVE Analysis for Threat Prioritization and Impact Prediction

The Common Vulnerabilities and Exposures (CVE) are pivotal information for proactive cybersecurity measures, including service patching, security hardening, and more. However, CVEs typically offer low-level, product-oriented descriptions of publicly disclosed cybersecurity vulnerabilities, often lacking the essential attack semantic information required for comprehensive weakness characterization and threat impact estimation. This critical insight is essential for CVE prioritization and the identification of potential countermeasures, particularly when dealing with a large number of CVEs. Current industry practices involve manual evaluation of CVEs to assess their attack severities using the Common Vulnerability Scoring System (CVSS) and mapping them to Common Weakness Enumeration (CWE) for potential mitigation identification. Unfortunately, this manual analysis presents a major bottleneck in the vulnerability analysis process, leading to slowdowns in proactive cybersecurity efforts and the potential for inaccuracies due to human errors. In this research, we introduce our novel predictive model and tool (called CVEDrill) which revolutionizes CVE analysis and threat prioritization. CVEDrill accurately estimates the CVSS vector for precise threat mitigation and priority ranking and seamlessly automates the classification of CVEs into the appropriate CWE hierarchy classes. By harnessing CVEDrill, organizations can now implement cybersecurity countermeasure mitigation with unparalleled accuracy and timeliness, surpassing in this domain the capabilities of state-of-the-art tools like ChaptGPT.

==> Figs/CVE2CWE.tex <==
\chapter{Automated Classification of CVEs to CWEs and to Vulnerability Types} \label{chapter_cve2cwe}
In this chapter, we discuss the importance of enriching CVE reports and propose a model on top of the pre-trained SecureBERT to automatically classify CVEs to CWEs. In addition, we introduce a new concept called Vulnerability Type (VT), that represent a group of CWEs that each VT represents particular set of characteristics. We also design another model to classify CVEs to VTs, where this classification plays an important role in CoA inference, discussed in Chapter \ref{sec: CoA}.

% -------------------------------------------
% ------------------------------------------- Introduction
% -------------------------------------------
\section{Introduction}
A cybersecurity vulnerability is any flaw in an information technology system, internal controls, or system procedures that attackers can exploit. Cyber attackers can gain access to the systems and acquire data through sources of vulnerability, and hence they are critical in the field of computer security. 
Unpatchable or Zero-day vulnerabilities are the major source of cybersecurity incidents, which can result in considerable economic losses for enterprises. 
The Common Vulnerabilities and Exposures (CVE) \cite{(2)CveMITRE2018} database is a repository of publicly disclosed information security vulnerabilities. CVE provides an easy and consistent means for vendors, companies, researchers, and other interested parties to communicate cybersecurity information. These reports are often low-level and product-oriented that typically fail to provide a high level insight about the underlying threats and therefore, they are not suitable for risk management and cyber threat intelligence. Thus, classifying existing vulnerabilities to hierarchically structured weakness enumerations (CWEs) \cite{(3)CweMITRE2018} is a key tool for understanding and mitigating the vulnerabilities. 
CWEs are designed in a hierarchical form, with weaknesses in lower levels inheriting the traits of their parents. Following this tree-based classification scheme is crucial since it reduces the prediction complexity and provides multi-level information about the threat that is useful in establishing a comprehensive understanding of the vulnerability.

Classifying CVE reports to  CWEs has previously been done manually, leaving dozens of critical and new CVEs unclassified, yet unpatchable. This significantly limits the utility of CVEs and slows down proactive threat mitigation, due to a scarcity of security experts and a growing number of vulnerability every day. 

Using cutting-edge text analytic and NLP technologies is critical for automating the process of CVE text reports since it demands a deep contextual analysis that traditional machine learning methods cannot provide. Pre-trained language models (LM), such as BERT, have lately received a great deal of interest from the research community for complex text analysis tasks. However, since these models are trained on generic English, they might be inefficient for processing domain-specific documents, such as CVEs. Thus, cybersecurity-specific LMs like SecureBERT can be a viable option for developing a robust and effective predictive model in cybersecurity.

In this chapter, we propose an automated method that uses to fine-tune the SecureBERT to classify CVEs to CWEs. We assessed the performance of our proposed model through using several testing methodologies and conducting a comparative research with other similar models to illustrate the efficacy and applicability of our approach. 

% -------------------------------------------
% ------------------------------------------- Problem Definition
% -------------------------------------------
\section{Problem Definition}

Cyber attacks enable malicious actors to break intended security policies by circumventing protective systems or influencing system resources or behavior. As a result, the attack leads in behavior that violates the victim's intended security regulations. Typically, attackers exploit a vulnerability by abusing an existing weakness in a system.
CWE is a hierarchically designed dictionary of software weaknesses for the purpose of understanding software flaws, their potential impacts if exploited, and identifying means to detect, fix, and prevent errors.
CWE classes are organized hierarchically, with higher level classes providing higher level attack characteristics and lower level classes inheriting the parent classes' features and adding micro granularity details. Therefore, determining the best path from a root to lower level nodes allows for the acquisition of fundamental and functional directions for detecting and analyzing the different properties of a vulnerability.

For example, given 'CVE-2004-0366: A \textit{SQL injection vulnerability} in the libpam-pgsql library before to 0.5.2 allows attackers to execute arbitrary SQL statements.', the description captures the attack action (execute arbitrary SQL statements) within a specific object (libpam-pgsql library) and specifies the consequence (SQL injection). While this low-level, product-oriented description depicts SQL injection exploitation, it falls short of clearly defining the characteristics of this malicious behavior, which is highly required to address possible prevention and/or detection measures. The supplementary CWE (CWE-89: SQL Injection) \footnote{https://cwe.mitre.org/data/definitions/89.html} gives high-level and non-product-specific information by addressing three critical questions: (1) why the attack is used: the system does not properly neutralize special elements; (2) how the attack is used: by changing the intended SQL query; and (3) what the probable results are: access or modify application data; and bypass protection mechanism.

The above-mentioned case is a confirmatory example to show how a CWE can paint a clear picture of the existing holes in the systems and reveals potential factors that cause vulnerability exploitation. Obtaining these factors is closely associated with the paradigm of pinpointing applicable mitigation or detection methods. For example, we can apply an "accept known good" input validation strategy, i.e., using a set of legit inputs that strictly 
conform to specifications and rejects the rest, to mitigate SQL injection. Besides, we can detect SQL injection by performing an automated static analysis (e.g., bytecode or binary weakness analysis), dynamic analysis (e.g., database or web service scanners), or design review (e.g., formal methods). 

\begin{figure}[!ht]
\includegraphics[width=1\textwidth]{Chapter 5/Chapter5_Figures/Hir.PNG}
\caption {It depicts the hierarchical representation of the CWEs. The red boxes show the CWE-89's relatives in the higher levels. This hierarchy plays an important role in understanding the character of the weaknesses in different level of details.} 
\label{fig:cwesnap}
\end{figure} 

Fig. \ref{fig:cwesnap} shows the hierarchical representation of the CWEs. Analyzing the path from the root all the way to any node in the lower levels is indispensable since each node reveals different functional directions to learn a weakness. For example, by tracking the path from the root node, CWE-707, to  CWE-89, we realize that the SQL injection (CWE-89) is a result of an improper neutralization of special elements in data query logic (CWE-943), where both weaknesses are associated with injection (CWE-74), and the injection itself is the result of improper formation and neutralization of a message within a product before it is read from an upstream component or sent to a downstream component (CWE-707). Incorporating this thorough knowledge graph helps to maintain countermeasures from different senses, even if the most fine-grain node is not available. For example, assume that only two coarse-grain candidates in different levels of hierarchy, CWE-707, and CWE-74, are available for CVE-2004-0366, while the most fine-grain weakness (CWE-89) is not discovered yet. Although fine-grain SQL injection characteristics is not exposed, investigating the coarse-grain candidates helps to find the common consequences and impacts, and accordingly extract defense actions against improper neutralization and injection (e.g., filtering control-plane syntax from all input). This example explicitly highlights the significance of the existing hierarchical structure of CWEs and shows how useful it is in perceiving the defense actions. 


A significant number of CVEs are currently mapped to a small set of CWE classes. Currently, about 70\% of the CWE classes have fewer than 100 CVEs about 10\% have no CVEs mapped to them, and only 10\% have more than 500 CVEs. The current approaches of classification work well only when a sufficient amount of data is available to train [10, 11, 12, 13].

\colorbox{orange}{Talk about NVD}

% -------------------------------------------
% ------------------------------------------- Related Works
% -------------------------------------------
\section{Related Works}
A great effort has been made initially by MITRE and NVD\footnote{National Vulnerability Database} to manually classify some CVEs to one or more CWE classes, each one shows critical shortcomings though.  Considering the growing number of CVEs and the high labor cost of manual classification, MITRE has classified 2553 CVEs (out of ~116K) to 364 CWE classes (out of 719) \cite{(3)CweMITRE2018}. On the other hand, NVD has \cite{(9)NVD2018} attempted to increase the quantity of CVE classification by mapping about 85,000 CVEs. Although MITRE has classified smaller number of CVEs compared with NVD, it considers a higher number of CWEs, and performs hierarchical and a more fine-grain classification. In the meantime, NVD classified more CVEs but it took smaller number of CWEs in to the account, without addressing the hierarchy. 

In the meantime, there have been several research efforts other than MITRE and NVD to analyze CVEs to enhance the searching process and to perform CVE categorization.
Neuhaus \textit{et al.}~\cite{(22)Neuhaus2010} proposed a semi-automatic method to analyze the CVE descriptions using topic models to find prevalent vulnerability types and new trends. The test result reports 28 topics in these entries using Latent Dirichlet Allocation (LDA) and assigned LDA topics to CWEs~\cite{(22)Neuhaus2010}. This approach shows very limited accuracy depending on the CWE type.

Na \textit{et al.}~\cite{(23)Na2016} proposed  Na\"ive Bayes classifier to categorize CVE entries into the top ten most frequently used CWEs with the accuracy of 75.5\%. However, the accuracy of this limited classification significantly decreases as the number of the considered CWEs increases (i.e., accuracy decreased from 99.8\% to 75.5\% when the number of CWE classes increased from 2 to 10). In addition, this approach does not consider the hierarchical structure for CWEs, which significantly limit its value.
Another classifier was developed to estimate the vulnerabilities in CVEs using the basis of previously identified ones by Rahman \textit{et al.} \cite{(24)Rehman2012}. This approach uses the Term Frequency-Inverse Document Frequency (TF-IDF) to assign weights to text tokens form the feature vector and Support Vector Machine (SVM) to map CVEs to CWEs. However, they use only six CWE classes and 427 CVE instances. In addition their classifier does not follow the hierarchical structure for CWEs as well. All these addressed issues and limitations are resolved in this work.

\colorbox{orange}{add few more}


% -------------------------------------------
% ------------------------------------------- Challenges
% -------------------------------------------
\section{Challenges}
Associating CVEs with CWEs allows cyber security researchers to understand the means, assess the impact, and develop solutions to mitigate threats. However, the problem is loaded with challenges. A CVE can be mapped to multiple and interdependent CWEs on the same route, creating uncertainty. On the other hand, there is a scarcity of high-quality mapping information since CVEs are presently mapped manually to CWEs, which is neither scalable nor reliable. Manual mapping of CVEs is not a practical strategy since new CVEs are introduced at a quick rate. Hence, effective approaches for automating the mapping of CVEs to CWEs are critical for addressing ever-increasing cybersecurity risks.

On the other hand, CVEs are typically short and low-level description written in an advanced language. The format and terminology used in these reports requires cybersecurity knowledge and a deep context understanding for automation. Traditional text mining approaches that work based on words frequency fail to adequately capture the context. On the other hand, the modern NLP tools and pretrained language models may not effectively and optimally process such advance language. Therefore, a domain-specific model that is trained on cybersecurity data is needed.

Furthermore, the available CVE-to-CWE dataset is highly unbalanced meaning that some CWEs are much more common than the others. A portion of this issue is justified, as NVD focuses on more general CWEs that encompass a broader range of specific characteristics, rather than using several distinct CWEs. For example, "CWE-79: Cross-site Scripting (XSS)" is the most frequently reported vulnerability in the NVD classification, accounting for 16,019 CVE reports. Meanwhile, NVD has only used a variant of the XSS vulnerability, the "CWE-87: Improper Neutralization of Alternate XSS Syntax" only one time. NVD's similar use of weaknesses to represent CVEs demonstrates that there are several primary CWEs that cover specific properties and can thus represent a large group of similar CWEs. 
However, this does not apply to all CWEs as some of them are not commonly exploited, yet carry unique properties. Therefore, there must be robust and well-defined approach to be able to classify CVEs to uncommon CWEs appropriately. Table \ref{fig:cwedist} shows the distribution of top 50 most commonly used CWEs by NVD. As depicted, the appearance of few CWEs such as "CWE-79: Cross-site Scripting (XSS)", "CWE-119: Improper Restriction of Operations within the Bounds of a Memory Buffer", and  "CWE-20: Improper Input Validation" is much higher than other weaknesses.

\begin{figure}[!ht]
\includegraphics[width=1\textwidth]{Chapter 5/Chapter5_Figures/CWEtop25_dist.png}
\caption {Shows the distribution of common CWEs } 
\label{fig:cwedist}
\end{figure} 
% -------------------------------------------
% ------------------------------------------- Methodology
% -------------------------------------------
\section{Methodology}
We addressed the issue of automatic CVE to CWE classification as a means of fine-tuning SecureBERT. We created a hierarchical classification layer on top of SecureBERT as a downstream task. This model takes a CVE description as input and returns corresponding CWE classes at each level of the hierarchy. To this end, we developed a top-down strategy, training a classifier on each node (class) in the CWE hierarchical tree. The classifier makes a choice for each node on whether to belong to a different sibling. The primary goal of this hierarchical structure is to direct the model's attention to the commonalities and contrasts between the sibling nodes.
This helps in lowering the model complexity by minimizing the number of output classes during the training procedure, as well as boosting model accuracy by allowing each classifier to focus on its children without being confused with other siblings' children. 
\iffalse
This contributes to model complexity reduction by limiting the number of output classes used during the training procedure, as well as model accuracy improvement by allowing each classifier to focus exclusively on its children without being confused by other siblings.
Therefore, to predict the relevant CWE class for a CVE, we track CWEs all the way down to the lowest possible level.
\fi
\begin{figure}[!ht]
\centering
\includegraphics[width=8cm]{Chapter 5/Chapter5_Figures/CWE_tree.png}

\caption {Shows the CWE tree structure. } 
\label{fig:CWE_tree}
\end{figure} 
Fig. \ref{fig:CWE_tree} shows the CWE's tree structure in advance and demonstrates the existing levels, and "Parent-Children" and "Sibling" relationships between the nodes. Tracing this tree from left, let's denote the $i_{th}$ CWE at Level $L$ by $c_i^{L}$ where $i\in\{1,...,N(c^{L})\}$ and $L\in \{1, ..., 7\}$. In our model design, for any given CVE, we aim to start predicting the associated CWEs from the $L=1$, and trace the CWE hierarchical tree for the correct class at each level to the node in the lowest possible level. Let's denote each CWE as a node $c_i^{L}$, and total number of CWEs at level $L$ with $N(c^{L})$. Let $G(c_i^{L})$ represents all the children of $c_i^{L}$:
% \begin{equation}
%     \textbf{G}(c_i^{L}) = \bigcup_{j=1} ^ K ~ c_j^{L+1} \text{~~~for~~~} K = {MIN~\Big{[} , \textbf{N}(\textbf{G}(c^{L}))~\Big{]}}
% \end{equation}
\iffalse
\begin{equation}\label{eq: child}
    \textbf{G}(c_i^{L}) = 
        \begin{cases}
                \bigcup_{j=1} ^ {\textbf{N}(\textbf{G}(c_i^{L}))} ~ c_j^{L+1} &,\,~~~ \textbf{N}(\textbf{G}(c_i^{L}))>0\\
                NULL & ,\,~~~ otherwise
        \end{cases}
        .
\end{equation}
\newline 

Eq. \ref{eq: child} returns the children of node $c_i^{L}$ if there is any, where $\textbf{N}(\textbf{G}(c_i^{L}))$ represents the number of children. It worth to note that, all the children of $c_i^{L}$ would take place in the next level of hierarchy $L+1$.
\fi

As initial step, we classify the given CVE to one or more $c_i^{L}$ and then as a next step, we only focus on the children of predicted parent $\textbf{G}(c_i^{L})$ and move forward until we reach the most fine-grain node possible (or desired).

We use the pretrained SecureBERT as the baseline model and add a multimodal classification layer on top. As depicted in Fig. \ref{fig: cve2cwe_model}, the model takes the CVE description tokenized by SecureBERT's tokenizer and pass it through the transformers stack and returns the embedding vector of first token ([CLS] token). In contrast to the hidden state vector associated with any other token, the hidden state associated with [CLS] is an aggregate representation of the entire input used for classification tasks.
This vector is connected to a pooling layer followed by a dense layer of size $N(L)$ returning the logits with no activation function, where $N(L)$ represents the total number of nodes in layer $L$. 

\begin{figure}
 \center
  \includegraphics[width=14cm]{Chapter 5/Chapter5_Figures/CVE2CWE_model.png}
  \caption{CVE to CWE hierarchical classification model design.}
  \label{fig: cve2cwe_model}
\end{figure}

In order to make the model works in a hierarchical form, we multiply the output logits with a given masking vector $MV$, and forward the results (final logits) to the decision making component. 
$MV$ is a sparse vector whose size equals to the initial output layer ($N(L+1)$) generated based on the predicted node in the previous level representing the predicted node's children. 
Assume, for an input CVE, the model classify it to node $c_i^{L}$. If the total number of nodes (aka, total number of possible CWE classes) in the next level $L+1$ equals to $N(L+1)$, $MV$ would be a vector of $0$s and $1$s in which, $1$s represent the indices of $c_i^{L}$'s children nodes in the level $L+1$, and $0$s refer to the non-children nodes. The initial value of $MV$'s elements in level $L=1$ would be all $1$s, since in the first round of training, there are only parents and children is defined. 
We multiply this vector to the initial output layer using element-wise multiplication to help the model recognizing which nodes it should be focusing on during training and backpropagation. In other word, this multiplications turns off the nodes which are not the children of previously predicted class, hence reducing the complexity by lowering the number of prediction classes for each input.

In addition to the hierarchical classification, we also define more general groups of CWEs, so-called vulnerability types. Following the MITRE guideline \footnote{https://github.com/center-for-threat-informed-defense/attack_to_cve/blob/master/methodology.md}, similar vulnerabilities often also have the same attack steps and accordingly similar properties in which, the similarity refers to the CVEs associated with similar CWE types. MITRE guideline defines 27 distinct vulnerability types without referring to the CWEs associated with each type. 
As mentioned earlier, CWEs have two sorts of relationship including parent-children and sibling. We leverage such relationships and manually map CWEs to their corresponding types. 
\begin{table}[ht]
    \Centering
    \scriptsize
    \begin{tabular}{|l |p{5cm}|p{6cm}|}
    \hline
        ID & \Centering{\textbf{Vulnerability Type}} & \Centering{\textbf{CWE ID(s)}} \\ \hline
        
       1 & General Improper Access Control & 284, 285, 287, 862, 863 \\ \hline
        
       2 & Improper Restriction of Excessive Authentication Attempts & 306, 307 \\ \hline
        
       3 & Authentication Bypass by Capture-replay & 294 \\ \hline
        
       4 & Overly Restrictive Account Lockout Mechanism & 645 \\ \hline
        
       5 & Use of Password Hash Instead of Password for Authentication & 836 \\ \hline
        
       6 & General Credential Management Errors & 255, 256, 257, 260, 261 \\ \hline
        
       7 & Cleartext Transmission of Sensitive Information & 319 \\ \hline
        
       8 & Hard-coded Credentials & 798 \\ \hline
        
      9 &  Weak Password/Hashing & 328, 916 \\ \hline
        
      10  & General Cryptographic Issues & 310, 324, 325, 326 \\ \hline
    11    & XML External Entity (XXE) & 611, 776 \\ \hline
        
      12  & XML Entity Expansion (XEE) & 776 \\ \hline
        
    13    & URL Redirection to Untrusted Site ('Open Redirect') & 601 \\ \hline
        
      14  & Cross-site Scripting (XSS) & 79, 692 \\ \hline
        
    15    & OS Command Injection & 78 \\ \hline
        
      16  & SQL Injection & 89, 564 \\ \hline
        
    17   &  Code Injection & 94 \\ \hline
        
      18  & Directory Traversal (Relative and Absolute) & 20, 22, 23, 24, 25, 26, 27, 28, 29, 30, 31, 32, 33, 34, 35, 36, 37, 38, 39, 40 \\ \hline
        
    19    & Symlink Attacks & 59, 61, 62, 64, 65, 73, 363 \\ \hline
        
      20  & Untrusted/Uncontrolled/Unquoted Search Path & 426, 427, 428 \\ \hline
        
    21    & Unrestricted File Upload & 434, 351, 436, 430, 73, 183, 184 \\ \hline
        
      22  & Deserialization of Untrusted Data & 502 \\ \hline
        
    23    & Infinite Loop & 835 \\ \hline
        
      24  & Cross-site Request Forgery (CSRF) & 352 \\ \hline
        
    25    & Session Fixation & 384 \\ \hline
        
      26  & Uncontrolled Resource Consumption & 400, 664, 770, 771, 779, 920, 1235, 410 \\ \hline
        
    27    & Server-Side Request Forgery (SSRF) & 918 \\ \hline
        
    \end{tabular}
    \caption{Mapping CWEs to vulnerability types.}\label{tab: cwe2vtype}
\end{table}

Table \ref{tab: cwe2vtype} shows our manual effort in mapping CWE to vulnerability types. Note that, vulnerability types are mainly defined for the purpose of finding CVEs with common set of techniques used to exploit that is useful in mapping CVEs to MITRE techniques. Therefore, such vulnerability types are not comprehensive and do not cover all existing CWEs. 


Fig. \ref{fig: cve2vt_model} shows the CVE-to-VT classification model architecture. It follows the similar structure as the hierarchical model with two main differences. First, it is a flat model and therefore, there is no masking vector. In addition, in decision making component, we utilize Softmax to maximize the probability of the predicted output. In short, output size of this multiclass classification model is the fixed number $27$ which equals to the total number of vulnerability types defined in Table \ref{tab: cwe2vtype}.

\begin{figure}[ht]
 \center
  \includegraphics[width=14cm]{Chapter 5/Chapter5_Figures/CVE2VT_model.png}
  \caption{CVE to CWE hierarchical classification model design.}
  \label{fig: cve2vt_model}
\end{figure}
% -------------------------------------------
% ------------------------------------------- Evaluation
% -------------------------------------------
\section{Evaluation}
In this section, we undertake a comparative evaluation of our proposed model's performance in classifying CVEs to CWEs using only human-readable language from CVEs.
We train two different classification models, a hierarchical CVE to CWE classification model and a CVE to vulnerability types classification model, and perform a comparative evaluation on each.
Additionally, we provide experimental settings for reproducing the model and discuss the model's strengths and drawbacks.

\subsection{Hierarchical CVE to CWE Classification Model}
For training the hierarchical model, we use a list of 63,481 CVE descriptions and classified them to one or more CWEs at each level of hierarchy. Note that, the lowest level CWE used by NVD is $L=5$ and therefore, we separately train five models corresponding to each level. 
For each model, we use Binary Cross Entropy (BCE) with logits as loss function for this multiclass multi-label classification task, and evaluate by the prediction accuracy and F1-score.  We use $10$ epochs with Adam optimizer and the initial learning rate of $3e-5$. For training each model at level $L+1$, we further fine-tune the trained model in level $L$ instead of raw pre-trained SecureBERT, to make sure it conveys the most recent information about CVE texts. In decision making component in the output layer of the model, we perform min-max normalization to produce a probability score corresponding to each output unit.

NVD dataset had classified 121,768 CVEs to 296 CWEs as of the date of authoring this article. However, there is a significant disparity in the frequency with which CWEs are used, indicating that some CWEs are significantly more prevalent than the others. This implies that infrequent CWEs are either rare or have characteristics in common with one of the frequent CWEs. 
As depicted in Table \ref{fig: TopCWE_dist}, $77.3\%$ ((94,176 CVEs)), $87.4\%$ (106,374 CVEs), and $93\%$ (113,211 CVEs) of the CVEs have been classified to top 25, 50, and 100 CWEs, respectively. Note that, in calculating true predictions, if the instance was originally labeled by more than one CWE (multilabel instances), and the model catches one with no false positives, it is considered correct classification because any correct prediction can lead to the correct label in the lower levels.

\begin{figure}
 \center
  \includegraphics[width=7cm]{Chapter 5/Chapter5_Figures/TopCWE_dist.png}
  \caption{Distribution of CWEs in CVE to CWE classification.}
  \label{fig: TopCWE_dist}
\end{figure}

\iffalse
There are 121,738 CVEs classified to 296 CWEs. 
top 25: 94,176
top 50: 106, 347
top 100: 113,211
\fi

In the hierarchical model, we classify CVEs to to top 25,  50, and 100 most common CWEs. We measure the performance of our proposed model using hit ratio and F1-score in the top K predictions defined as follows:

$$
\text{Hit Ratio at K (HR@K)} = \frac{P^{K}_{hit}}{P_{all}}
$$
$$
\text{F1-Score at K (F1@K)} = \frac{P^{K}_{hit}}{P^{K}_{hit} + P^{K}_{fail}}
$$
Where HR@K represents the harmonic average classification accuracy for which the correct answer is included in the top K prediction, and F1@K denotes the harmonic average F1-score when the correct classification includes in the top K prediction. In this context, $N^{K}_{hit}$ refers to the number of times we hit the for which the correct answer is included in the top K predictions, $N^{K}_{fail}$ specifies the number of samples for which the correct answer is not included in the top K predictions, and $P_{all}$ denotes the total number of the samples in the dataset.
\begin{table}[!ht]
\centering
 \caption{SecureBERT performance evaluation on hierarchical classification of CVEs to top 25, 50, and 100 CWEs.}
 \label{tab: cve2cwehir_eval}
\subcaption*{Top 25 CWEs}
\begin{tabular}{|l|c|c|c|c|c|c|c|}
 \hline
%  \multicolumn{4}{c}{Balanced Class Prediction} \\
%  \hline
 L& No. CWEs &\textbf{HR@1} & \textbf{F1@1} & 
 \textbf{HR@2} & \textbf{F1@2} &
 \textbf{HR@3} & \textbf{F1@3}\\
 \hline
 1 & 8 & 91.80 & 91.11 & 96.82 & 95.92 & 98.92 & 98.55\\
 2 & 18 & 94.55 & 91.38 & 94.95 & 92.44 & 95.11 & 92.63\\
 3 & 14 & 97.51 & 96.08 & 97.51 & 96.16&97.51 & 96.16\\
 4 & 6 & 95.22 & 94.35 & 95.42 & 94.39 & 95.61 & 95.09\\
 \hline
 \end{tabular}
 \bigskip
\subcaption*{Top 50 CWEs}
 \begin{tabular}{|l|c|c|c|c|c|c|c|}
 \hline
  L & No. CWEs & \textbf{HR@1} & \textbf{F1@1} & 
 \textbf{HR@2} & \textbf{F1@2} &
 \textbf{HR@3} & \textbf{F1@3}\\
 \hline
 1 & 8 & 91.24 & 91.15 & 95.91 &93.59 & 98.18 & 95.77\\
 2 & 30 & 93.57 & 87.48 & 94.29 & 89.63 & 94.33 & 91.52\\
 3 & 36 & 95.46 & 85.89 & 95.26 & 88.96 &95.26 & 88.96\\
 4 & 13 & 94.02 & 85.21 & 94.73 & 85.37 & 94.73 & 85.37\\
 5 & 3 & 91.53 & 91.53 & 91.53 & 91.53 & 1.0 & 1.0\\
 \hline
 \end{tabular}
  \bigskip
\subcaption*{Top 100 CWEs}
 \begin{tabular}{|l|c|c|c|c|c|c|c|}
 \hline
  L & No. CWEs &\textbf{HR@1} & \textbf{F1@1} & 
 \textbf{HR@2} & \textbf{F1@2} &
 \textbf{HR@3} & \textbf{F1@3}\\
 \hline
 
 1 & 9 & 90.77 & 90.31 & 95.12 & 93.97 &97.51 & 95.36 \\
 2 & 43 & 91.11 & 85.89 & 92.30 & 87.35 &92.30 & 87.35\\
 3 & 63 & 94.24 & 84.91 & 94.61 & 85.17 &94.61 & 85.17\\
 4 & 27& 94.57 & 90.81 & 95.44 & 92.25 & 95.44&92.25\\
 5 & 7 & 90.80 & 90.96 & 91.11 & 90.99 & 91.11 & 91.07\\
 \hline
 \end{tabular}
\end{table}

Table \ref{tab: cve2cwehir_eval} shows the performance of the proposed hierarchical model in classifying 25,915 CVEs to top 25, 50, and 100 CWEs in different levels of hierarchy. Each table shows the hit ratio and F1-Score in top K (HR@K and F1@K) predictions for each level of hierarchy, as well as the number of CWE classes exist at each level. In essence, given the CWE information of a CVE at level $L$, the table shows the model's prediction performance at $L+1$.
In classifying CVEs to top 25 CWEs, which covers the majority of CVEs, our model successfully classified CVEs to the correct CWEs with the hit ratio ranged from 91.8\% up to 98.92\%, and F1-score between 91.11\% and 98.55\%, with K$\in \{1,2,3\}$ in different levels. Despite the promising performance in classifying CVEs to top 50 and 100 CWEs, lower performance (particularly in F1-scores) compared to top 25 can be justified by two reasons. First, the additional CWE classes have much lower number of CVEs in the training set causing less accurate prediction, Furthermore, many of such additional CWEs share common characteristics with the frequent CWEs and as a result, CVEs are mostly mapped to the common ones by NVD. Therefore, as we use such mappings as labels in our training set, our model tends to classify CVEs that originally associated with uncommon CWEs to frequent CWEs instead.

The hierarchical model offers the researchers a variety level of classification granularity. In other words, different levels of information may be required by researchers to characterize the properties of CVEs. As a result, providing level-specific knowledge about CVEs can offer various aspects of CVE characteristics. CVEs, on the other hand, may exploit more than one weakness, which cannot be addressed if they are mapped to only one CWE. As an outcome, hierarchical models are highly functional in recognizing such weaknesses and providing broader insight into exploit to help in better assessment and, consequently, defense planning.
\iffalse
For example, in a vulnerability assessment study, one may seek to know general type of the weakness for  
\fi
\subsection{CVE to Vulnerability Type (VT) Classification Model}
Similar to individual CWEs, VTs are  not distributed uniformly in NVD dataset. As depicted in Fig. \ref{fig: TopVT_dist}, about $72.3\%$ (41,240) and $88.03\%$ (50,174) of the CVEs are associated with top 5 and top 10 VTs, respectively. In addition, four VT IDs including 4, 5, 9, and 20 do not have any corresponding CVE in the NVD dataset. For training the CVE to VTs, we use $70\%$ of the available CVE descriptions to classify them to one of the top 5, 10, and all 23 VTs provided in Table \ref{tab: cwe2vtype}.
\begin{figure}
 \center
  \includegraphics[width=10cm]{Chapter 5/Chapter5_Figures/VT_dist.png}
  \caption{Distribution of CWEs in CVE to CWE classification.}
  \label{fig: TopVT_dist}
\end{figure}


\begin{table}[ht]
\centering
 \caption{SecureBERT performance evaluation in classifying CVEs to top 5, 10, and all vulnerability types.}
 \label{tab: cve2vt_eval}
\begin{tabular}{|l|c|c|c|c|c|c|c|}
 \hline
 L & \textbf{HR@1} & \textbf{F1@1} & 
 \textbf{HR@2} & \textbf{F1@2} &
 \textbf{HR@3} & \textbf{F1@3}\\
 \hline
 Top 5 &93.12  & 91.88 & 95.21 & 92.59 & 96.34 & 93.23\\
  Top 10 &  91.66 & 89.28 & 93.71 & 91.44 & 95.07 & 92.68\\
   All & 87.53 & 84.32 & 90.35 & 86.64 & 91.26 & 87.19\\
 \hline
 \end{tabular}
 \end{table}
Table \ref{tab: cve2vt_eval} shows the performance of our model. 

\iffalse
NVD has classified some CVEs to \textit{Categorical CWEs} or \textit{Others}, not any specific CWE ID. Excluding such CVEs, our training dataset contains $64,490$ CVE reports. We also use Binary Cross Entropy (BCE) with logits as loss function for this multiclass multi-label classification task. We evaluate the model at each level and in total using accuracy and F1-score.
We also provide partial accuracy measure which represents the rate of prediction even if there is a false prediction among trues. This is important since any instance with false positive in prediction might be properly predicted in level $L=L+1$, if passed from $L$. In calculating regular accuracy, if the instance was originally labeled by more than one CWE (multilabel instances), and the model catches one with no false positives, it is considered correct classification because any correct prediction can lead to the correct label in the lower levels. The F1 score is also considered in a similar justification.

For training, we used $6$ epochs with Adam optimizer and the initial learning rate of $1e-5$. The confidence value for considering a class a true prediction in the first level is $\tau=0.45$ and for the other lower layers is $\tau=0.9$. In table \ref{tab: cve2cwe_eval}, we report our classification performance and compare the prediction results with other similar models such as RoBERTa (base) and SciBERT using $27,412$ testing instances. 
\begin{table}
\centering
\begin{tabular}{l|c|c|c}
 \hline
%  \multicolumn{4}{c}{Balanced Class Prediction} \\
%  \hline
 \textbf{Model}&\textbf{Partial Accuracy} & \textbf{Accuracy} &  \textbf{F1-score}\\
 \hline
  RoBERTa &  88.38  &  86.54  & 84.01 \\
  SciBERT  &  88.41  &  84.63  & 82.77\\
  SecureBERT &  X  &  X  & X\\
 \hline
 \end{tabular}
 \caption{SecureBERT performance evaluation on CVE to CWE hierarchical classification}
 \label{tab: cve2cwe_eval}
\end{table}
The evaluation result shows SecureBERT outperforms the similar models in this classification task.
\section{Conclusions and Future Works}
In this work, we made the following contributions:
\begin{enumerate}
    \item Manually categorize to similar CWE to different categories known as vulnerability types where each category represent particular set of behaviors and impacts.
    
    \item design a neural network classifier on top of SecureBERT that can hierarchically analyze and classify CVE's textual description according to the CWE tree.
    
    \item provide a comparative evaluation of the work and show its effectiveness 
    
\end{enumerate}
\fi

==> Figs/CVSS.tex <==
\chapter{Automated CVSS Prediction}

% -------------------------------------------
% ------------------------------------------- Introduction
% -------------------------------------------
\section{Introduction}
The Common Vulnerability Scoring System is a free and open industry standard for measuring the severity of security vulnerabilities. This provides a way to capture the principal characteristics of a vulnerability and produce a numerical score reflecting its severity. The numerical score can then be translated into a qualitative representation (such as low, medium, high, and critical) to help organizations properly assess and prioritize their vulnerability management processes. 

Currently, the CVSS is calculated through manual engineering effort that is expensive, inefficient, inconsistent, and problematic. The NIST's security experts take days or even longer to analyze CVEs and measure their severities such that many CVEs may remain indeterminate. This controversial cycle simply means cybersecurity analysts cannot rely on the availability of perpetual severity metrics for every CVEs. Thus, they are limited to available CVE elements such as description to focus. 

Therefore, mimicking the expert thinking and automating the entire scoring procedure is the ultimate solution to tackle this manual prediction problem. With this aim in mind, the automatic prediction of CVSS score is beneficial in CVE characterization from two points of view. First, it helps to prioritize vulnerabilities for threat analysis and risk management. Second, extracting different CVSS factors means obtaining new characteristics of CVEs which might help discover an appropriate defense action. 

% 
When it comes to properly documenting the features and severities of software vulnerabilities, CVSS is the standard protocol, which has been issued in two versions, with CVSS V2, and CVSS V3 (and CVSS V3.1) \footnote{https://www.first.org/cvss/} both being extensively utilized in the computer security domain.  
Both CVSS versions are structured similarly, with a series of multiple-choice questions to the vendors concerning the vulnerability and classified into three groups: base, temporal, and environmental. The base group defines the inherent properties of the vulnerability, the temporal group defines how those properties vary over time, and the environmental group illustrates the severity of a vulnerability in the context of a particular organization. We will concentrate on CVSS V3 in this work as it is newer and broadly applied recently than the former version.


\begin{table}
\small
\centering
 \begin{tabular}{|l | l | l |} 
  \hline
 \multicolumn{3}{c}{\textbf{CVSS V3}} \\
  \hline
  \hline
   \multicolumn{1}{|c|}{\textbf{Base Vector}} & \multicolumn{1}{|c|}{\textbf{Temporal Vector}} & \multicolumn{1}{|c|}{\textbf{Environmental Vector}}\\
   \hline
  Attack Vector (AV) &  &\\
  Attack Complexity (AC) &  &Modified Base Metrics (M*)\\
  Privileges Required (PR) & Exploit Code Maturity (E) & Confidentiality \\
  User Interaction (UI) & Remediation Level (RL)& Requirement (CR)\\
  Confidentiality (C) & Report Confidence (RC)   &Integrity Requirement (IR) \\
  Availability (A) & & Availability Requirement (AR)\\
  Integrity (I) & & \\
  Scope (S) &  &\\
   \hline
\end{tabular}\hfil
     \caption{\label{tab: CVSSV3} The resources collected for cybersecurity textual data}
\end{table}

Table \ref{tab: CVSSV3} shows the different fields required by CVSS V3. When all responses about a vulnerability have been completed, they are merged using a common syntax to form a CVSS Vector. Each CVSS version has a non-linear severity formula that accepts all data as input and delivers a severity value between 0.0 and 10.0.
Since this equation is not linear, slight changes in the vector can result in significant variances in the severity score. CVSS V3 and V3.1 have the same fields and differ solely in the severity algorithm, which affects a small number of vulnerabilities. In the rest of our work we use the term "CVSS V3" to describe both the CVSS V3 and V3.1 specifications. In addition, since  Temporal and Environmental vectors are derivable from Base Vector, we only process the Base vector, which consists of eight different metrics including \textit{Attack Vector (AV)}, \textit{Attack Complexity (AC)}, \textit{Privileges Required (PR)}, \textit{User Interaction (UI)}, \textit{Confidentiality (C)}, \textit{Availability (A)}, \textit{Integrity (I)},  and \textit{Scope (S)}. Each metric also can get different values which is demonstrated in Table \ref{tab: CVSSV3_base}. Our target in this work is to automatically predict the value of each eight metrics for a given vulnerability using the corresponding CVE ID description, utilizing pretrained SecureBERT language model.

\begin{table}
\small
\centering
 \begin{tabular}{|l | l |} 
\hline
 \multicolumn{2}{c}{\textbf{CVSS V3 Base Metric}} \\
  \hline
  \hline
   \multicolumn{1}{|c|}{\textbf{Metric}} & \multicolumn{1}{|c|}{\textbf{Values (classes)}} \\
   \hline
  Attack Vector (AV) & Network (N) | Adjacent (A) | Local (L) | Physical (P) \\
  \hline
  Attack Complexity (AC) & Low (L) | High (H) \\\hline
  Privileges Required (PR) & None (N) | Low (L) | High (H) \\\hline
  User Interaction (UI) & None (N) | Required (R)\\\hline
  Confidentiality (C) & None (N) | Low (L) | High (H) \\\hline
  Availability (A) & None (N) | Low (L) | High (H)\\\hline
  Integrity (I) &  None (N) | Low (L) | High (H)\\\hline
  Scope (S) & Unchanged (U) | Changed (C) \\
   \hline
\end{tabular}\hfil
     \caption{\label{tab: CVSSV3_base} Shows the CVSS V3 Base metrics and the potential values.}
\end{table}

% The base score metrics and the factors within each are depicted in Fig.~\ref{fig:CVSSv3_metrics}.
% \begin{figure}
% \centerline{\includegraphics [width=1\textwidth]{Chapter 4/Chapter4_Figures/CVSSv3_metrics.png}}
% \caption {CVSS 3 structure}
% \label{fig:CVSSv3_metrics}
% \end{figure}

\section{Problem Definition}
For security analysts such as NIST's, it typically takes days or weeks to assess and annotate vulnerabilities that results in huge number of unprocessed vulnerabilities which have been publicly disclosed for a long time. Therefore, relying solely on metadata provided by databases such as NVD to analyze and prioritize vulnerabilities is not practical and researchers must focus on early available piece of data at the time of disclosure such as human readable description and possibly public references like vendor reports.

Such a manual procedure is costly, and a real-time threat evaluation of new vulnerabilities necessitates a large amount of labor due to the growing number of disclosed vulnerabilities every day; thus, it would be more affordable to organizations if it could be automated, which consequently allows timely manner and intuitive defense planning including security policy reconfiguration, limiting access, and/or shutting them down while waiting for a remediation to be applied, all based on the severity of the vulnerability. 
In this work, we propose an automated system that uses the free-form text descriptions of disclosed vulnerabilities to predict the CVSS base vector of these vulnerabilities and then we discuss the shortages of automating CVSS prediction procedure.

% -------------------------------------------
% ------------------------------------------- Related Works
% -------------------------------------------
\section{Related Works}
To the best of our knowledge, there are only a few efforts in automating CVSS prediction in recent years. Khazaei \textit{et al}~\cite{khazaei2016automatic} introduced an objective method for CVSS V2 score calculation by extracting textual features from CVE descriptions and employing SVM, Random Forest, and fuzzy systems for prediction. In this study, the descriptions are tokenized, and after performing standard text mining preprocessing such as filtering the stop-words and stemming, the TF-IDF score of words is calculated, and the dimension is reduced using PCA and LDA techniques. The CVSS V2 scores are roughly predicted within the interval of $[i,i+1)$ where $i\in\{0,1,2,...,9\}$. This works reported $88.37\%$ accuracy through testing the fuzzy system implementation. This work leveraged an off-the-shelf machine learning model and failed to consider and report many important metrics in CVSS prediction. This work exclusively focused on finding the direct relationship between CVE description and the final score, while original scores are calculated based on different CVSS metric values where each metric specifies a variable in the non-linear score calculation formula. This binary method performs as a classification task which is problematic since one word (feature) might have a different impact on each metric, and training every metric in one shot is error-prone.
In the meantime, the bag-of-word approach does not take the context and semantic into account and cannot handle potential unseen entries in to-be-announced CVE reports, such as synonym words and abbreviations.
In addition, there is no evidence showing the performance of this tool in predicting different classes since different classes have a different number of samples, and predicting scores for those who have less number of samples is important. 

In a similar approach, Elbaz \textit{et al}. \cite{elbaz2020fighting} implemented another technique based on linear regression to automatically predict the CVSS vector of newly disclosed vulnerabilities using their textual description. They used a similar bag-of-word approach and represented each CVE by word frequency vector. After filtering stop-words, two different dimension reduction approaches applied to select the most predictive features from the corpus. In the first approach, the software vendor, product name, and software target exist in the Common Platform Enumeration (CPE), and all the words in CWE titles are collected, and a white-list is generated to find and discard irrelevant features. In the second approach, the conditional entropy score for each word associated with each CVSS metric is calculated, and the top N words with the lowest score are selected for evaluation. Then a linear regression model is created to predict the scores for each CVSS metric. The accuracy of predicting each metric is varied from $60\%$ to $95\%$. This study suffers from certain weaknesses. 
First, similar to the previous work, the features are limited to the keywords extracted from CVE reports and CWE titles. This corpus fails to cover context and accordingly, semantic features such as synonyms, abbreviations, and similar words. Hence, there might be some less frequent words uniformly distributed among different values of one metric with a strong relationship with other words, which is a key signature for one specific value. The addressed feature extraction method in this study cannot find such a relationship, and therefore, it will assign a high entropy score to this word, and it will automatically be ignored in the classification. In addition, limited corpus without semantic feature analysis may not handle a new word or different writing standard, which is very likely to face since different vendors have a different writing style and new concepts might be raised in the future CVE description.
In addition, the evaluation is incomplete and failed to address some important points. About half of the metrics are imbalanced, which means that the frequency of instances for one metric is much higher than the others. E.g, in \textit{Attack Vector}, there are $\sim35K$ instances with \textit{Network} value, while there are less than $500$ samples with \textit{Physical} value out of $43,000$ existing labeled CVEs. This can easily lead to overfitting during training that this study did not address. 


% -------------------------------------------
% ------------------------------------------- Challenges
% -------------------------------------------
\section{Challenges}
Automating CVSS score prediction is a challenging task. The existing works are limited, or build upon imprecise assumptions. Predicting the CVSS score requires deep analysis of each element in the vectors and therefore, a direct approach to obtain the final severity score would be problematic since any small mistake may compromise the entire output significantly. Instead, dividing the CVSS to smaller elements and approaching the problem gradually would provide multi-level information about the vulnerability (each metric provides unique threat behavior). This would become even more important since it is proven that vulnerability descriptions often do not provide enough information about the entire threat characteristics, so any partial information about the threat would be beneficial in case the automated model cannot provide an exact final severity score.

On the other hand, traditional information extraction methods and machine learning algorithms may not be the most effective approach to tackle this problem. Such methods mainly work based on statistical analysis and word frequency, treating the available text as a bag-of-word. This strategy is unable to adequately capture the context and extract semantic relationships throughout the text, leading to missing important information and consequently a non-robust predictive model. 

Our training dataset comprises CVE descriptions whose CVSS vector is already assigned by NVD. In other words, each CVE in this dataset contains a CVSS base metric vector. This dataset is highly unbalanced, which implies that the frequency distribution of a specific value within each metric may highly different than the others.
Existing works failed to adequately address imbalance data problem and did not provide detailed performance evaluation regarding this issue in CVSS dataset. 
Table \ref{fig: metric_dist} shows the value distribution within each metric. 
\begin{figure}
\centerline{\includegraphics [width=13cm]{Chapter 4/Chapter4_Figures/CVSS_dataset.png}}
\caption {Numbers of available labeled records in each value for each CVSS metric. This shows the imbalance data problem in CVSS dataset}
\label{fig: metric_dist}
\end{figure}

% -------------------------------------------
% ------------------------------------------- Model Design
% -------------------------------------------
\section{Model Design}
In this section, we present our CVSS vector prediction pipeline. Since there are eight metrics, we train eight individual models, in which, in each model the input is the CVE description of a vulnerability and the output is the predicted value for the target metric. A general overview of the proposed CVSS analysis pipeline is depicted in Fig. \ref{fig: cvss_model}.
We utilized the pre-trained SecureBERT as the baseline and added an extra TF-IDF module to help the model processing the imbalance data. In this architecture, the model takes the CVE description, tokenize it using SecureBERT's BPE tokenizer and pass it through the transformer layers. Then, the [CLS] token vector representation is passed through a pooling layer and the output vector is merged with another vector (tensor) that represents the customized TF-IDF vector of the same CVE description. At the end, the merged vector is connected to the final dense layer (feed forward neural network) that its size equals to the number of potential values in the metric of interest.
\begin{figure}
 \center
  \includegraphics[width=12cm]{Chapter 4/Chapter4_Figures/CVSS_model.png}
  \caption{CVSS metric value prediction model design. For each CVSS metric, there is a separate model that is trained independently.}
  \label{fig: cvss_model}
\end{figure}


\noindent\textbf{TF-IDF Module}--\\
As mentioned earlier, CVSS data is highly unbalanced and to reduce the impact of this imbalancity during the training, we utilize a customized TF-IDF module that generates word-frequency based vectors, representing the input data with respect to the minority classes (values) in models corresponding to each metric. In a nutshell, according to our investigations, if we consider each potential value within each metric as a class, there are some words, so-called signature words, that are frequently appear in minority classes. For example, in CVEs whose the value of \textit{Attack Vector (AV)} metric is \textit{Adjacent Network (A)}, words like "adjacent", "Bluetooth", "pairing", and "dongle" are frequently appeared in the description. In another example, when the value of \textit{Attack Complexity (AC)} is \textit{High (H)}, "man-in-the-middle", "memory-cache", "padding", and "prolog" are frequently observed. 
On the other hand, keyword matching for predicting the value would not be an effective approach as these words are not uniquely appear in one specific class. In addition, when the training data is not large enough, even a powerful language model will not be able to learn the context and semantic relationships sufficiently. 

TF-IDF~\cite{ramos2003using} is an effective method in text mining to identify words that frequently appear in a particular class and rarely or never occur in other classes. 
Here, we aim to provide an external hint to the model to help recognizing the minority classes during the training using TF-IDF score, to extract signature words and convert them to a vector to merge with SecureBERT's output. Our assumption is that an extra emphasizes on important yet infrequent signature words during the training would benefit the model to adjust its weights to better recognize minority class(es). To recall, class refers to each value within a metric.

% 
In this context, we first conduct the standard text cleaning steps on our training set such as removing stop words, special characters, punctuations, and numbers, perform stemming, and then within each metric, we tokenize all reports belong to minority class and create a dictionary of words. Then, we calculate the the TF-IDF score of each word in this dictionary against all classes. In other words, if metric \textit{M} contains \textit{n} different classes, every words in the dictionary is represented by \textit{n} TF-IDF score, each corresponds to an individual class in a vector of size \textit{n}. This vector then is normalized to re-scale the scores to a range of 0 to 1. These normalized values represent the statistical relevance of a term belonging to a class, with values closer to 1 indicating higher importance. Since we aim to only identify minority classes using TF-IDF score vectors, we implement a filtering procedure based on a hyperparameter threshold to select words whose scores are in minority class(es) are "significantly" higher than their scores in majority classes. As a results, every vulnerability description  is defined by a set of \textit{q}-dimension TF-IDF vector if it shares any word with minority class word dictionary, where \textit{q} refers to the number of existing classes in metric \textit{M}. Then, we take the average of these vectors as the final TF-IDF vector representation of the input description. Table \ref{fig: TF-IDF_schema} shows the high level overview of TF-IDF vector creation.
\begin{figure}
 \center
  \includegraphics[width=15cm]{Chapter 4/Chapter4_Figures/TF-IDF_schema.png}
  \caption{Shows the different steps in generating customized TF-IDF vectors to represent CVE descriptions.}
  \label{fig: TF-IDF_schema}
\end{figure}

Let $\delta(M)$ be the dictionary of terms in minority class(es) in metric $M$:
\begin{equation}
    \delta(M) = \{w_1, w_2, ..., w_r\}
\end{equation}

If $M=\{c_1, ..., c_q\}$ represents the existing classes in metric $M$, for each $w \in \delta(M)$, we return $q$ scores (TF-IDF scores) corresponding to each $c \in M$:
\begin{equation}
    T(w, M)= [t^w_{c1}, ...,t^w_{cq}].
\end{equation}

Then we normalize each vector $T(w_i, M)$ by dividing all elements by the maximum value of the vector as $MAX[T(w_i, M)] + \epsilon$ ($\epsilon$ is a small number added to avoid divide by zero)and call it $T'(w_i, M)$.

% Let $\mathcal{T}$ be the set of TF-IDF vectors $T'(w_i, M)$ for all words in $\delta(M)$ as follows:
% \begin{equation}
% \label{eq: tfidf_norm}
%     \mathcal{T}(M) = \bigcup T'(w_i, M),\forall w_i \in \delta(M)
% \end{equation}

Here, our target is to provide a secondary representation of the input text beside SecureBERT's output, by conducting a statistical analysis to find those terms which are highly likely to appear in minor classes and rare in other classes. This vector representation will be concatenated by the SecureBERT's output and yield to the classification layer together. Therefore, given $T'(w, M)$, we first define a probability threshold $0<th<1$. Then,  for each $T'(w_i, M)$, we make sure one element corresponding to a minority class is greater than threshold ($t^w_{i,fj} > th$) and the remaining elements are smaller than $1-th$. In other words, we compare all \textit{q} number of TF-IDF scores associated with each word with the threshold and identify those  whose value corresponding to a minority class is significantly higher than other classes (according to the threshold).  Any word that satisfies both conditions will be added to the signature term dictionary $Dict(M)$ corresponding to each metric. Therefore, $Dict(M)$ contains words which are highly informative about minority values within each metric.

For any training input CVE description within each metric prediction model, we check how many terms it shares with $Dict(M)$. Let $S=\{w'_1, ...,w'_n\}$ represent the terms in a CVE description, and $g(S, M)=S \cap Dict(M)$ be the set of shared terms between $S$ and $Dict(M)$. For any term $w'\in g(S, M)$, we retrieve the TF-IDF vectors using Eq. \ref{eq: tfidf_norm} and take the average of all vectors to construct the TF-IDF representation of the CVE:
\begin{equation}
    \mathcal{V}(S, M) = Mean (T'(w', M)), \forall w'\in g(S)
    \label{eq: tfidf_norm}
\end{equation}

$\mathcal{V}(S, M)$ is a vector with a size equal to the number of values within a metric representing the probability score of a CVE being associated with each value, with respect to the signature words. Since signature words are extracted from minor classes, the vector elements associated with the dominant class samples are quite often zero or close to zero, indicating that this vector represents the chances that a CVE is associated with minor value, if the CVE shares any words with the signature word dictionary $Dict(M)$; otherwise, all elements would be zero.
% -------------------------------------------
% ------------------------------------------- Evaluation
% -------------------------------------------
\section{Evaluation}
In this section, we conduct a comparative evaluation on the performance of our proposed model in predicting the value of each metric separately, based only on CVE human-readable text. We also provide the experimental settings for the purpose of reproducing the model, and discuss the advantages and limitations of the model as well as some suggestions to improve the effectiveness of the CVSS prediction automation.
\\

\noindent\textbf{Experimental Settings}\\
We used NVD dataset that contains 41,447 CVEs reports that each is assigned by a CVSS vector for training the proposed model. For each report, we create two vector representations, a word vector representation generated by the SecureBERT's tokenizer, and a customized TF-IDF vector utilizing the methodology discussed in the previous chapter. In addition, we conduct data resampling  for minority class(es) within each metric by randomly duplicating samples, to reduce the impact of imbalance data problem and avoid overfitting while training. We train the model through 10 epochs with mini-batch size of 12 with a learning rate equal to $1e-5$. The training objective is to minimize the $Cross Entropy$ error using $Adam$ optimizer. \\
% In a 

\noindent\textbf{Model Performance}\\
Table \ref{tab: cvss_results} shows the comparative performance of our model in predicting each eight values in the CVSS base metric vector, using testing dataset of $5,357$ (20\% of the main dataset) CVE reports. We evaluated two version of model, one with and one without the TF-IDF module. This table shows the accuracy and the F-1 score in both micro and macro level. Considering the shortage of key information in CVE reports and imbalance class problem, SecureBERT achieved $80\%-96\%$ prediction weighted accuracy, $80\%-95\%$ micro-level and $73\%-91\%$ macro-level F1-score.

\begin{table*}
\centering
\scriptsize
 \begin{tabular}{|c |c |c| c | c | c |c | c |c | c |} 
  \hline

%   \hline
   Model & Metric & {AV} & {AC} & {PR} & {UI} & {S} & {C} & {I} & {A} \\
  \hline
SecureBERT & Accuracy & {\textbf{89.57}} & {\textbf{96.04}} & {\textbf{80.59}} & {\textbf{93.01}} & {\textbf{94.60}} & {83.23} & {84.35} & {\textbf{87.40}} \\

with & F1-Score (Micro) &{\textbf{89.45}} & {\textbf{95.96}} & {\textbf{80.58}} & {\textbf{93.01}} & {\textbf{94.39}} & {\textbf{83.23}} & {84.35} & {\textbf{87.04}} \\

TF-IDF & F1-Score (Macro) & {\textbf{76.16}} & {\textbf{81.10}} & {\textbf{73.67}} & {\textbf{91.35}} & {\textbf{89.91}} & {\textbf{80.70}} & {83.58} & {\textbf{72.47}} \\
\hline
% -----------------------------------------------------------------------------------------
 SecureBERT & Accuracy & {89.52} & {95.85} & {79.42} & {91.78} & {92.06} & {\textbf{83.25}} & {\textbf{84.99}} & {86.01} \\
 
 without & F1-Score (Micro)  &{89.38} & {95.84} & {79.42} & {91.78} & {92.06} & {83.21} & {\textbf{84.59}} & {85.91} \\
 
 TF-IDF  & F1-Score (Macro) & {75.54} & {80.34} & {72.03} & {89.21} & {86.88} & {80.37} & {\textbf{83.83}} & {71.41} \\
              
%     \hline
%     RoBERTa  & Accuracy & {AV} & {AC} & {PR} & {UI} & {S} & {C} & {I} & A \\
%     with  & F1-Score (Micro) &{AV} & {AC} & {PR} & {UI} & {S} & {C} & {I} & A \\
%   TF-IDF  & F1-Score (Macro) &{AV} & {AC} & {PR} & {UI} & {S} & {C} & {I} & A \\

    \hline

\end{tabular}\hfil
     \caption{\label{tab: cvss_results} CVSS value prediction results}
\end{table*}
According to the performance results, the model with TF-IDF module outperforms the other model indicating the effectiveness of this module in identifying the correct class when the corresponding classes regularly contains specific key words. Meanwhile, at first glance, the difference between micro and macro metrics reveals the impact of the unbalanced data problem in metrics with a greater incidence of unbalance. However, prediction result of some metrics whose micro-macro performance gap is small, yet unbalanced, such as \textit{User Interaction (UI)} and \textit{Scope (S)}, shows the proposed model could successfully identify the correct class. This implies that the CVE reports typically provide required information for these metrics. On the other hand, the high rate of false positives in both minor and dominating values of some metrics such as \textit{Confidentiality (C)} and \textit{Availability (A)} indicates the lack of key knowledge in CVE reports, leading to lower rate of correct prediction. Table \ref{tab:cvss_confmatrix} shows the confusion matrix of each eight individual models.


\begin{table}[!ht]
\Centering
\footnotesize
\begin{tabular}{cc|cc cc cc}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{4}{c}{{\footnotesize \textit{Predicted}}} \\ 
\multicolumn{1}{c}{\textbf{\textcolor{CadetBlue}{AV}}} & 
\multicolumn{1}{c|}{} & 
\multicolumn{1}{c}{N} & 
\multicolumn{1}{c}{L} &
\multicolumn{1}{c}{A} & 
\multicolumn{1}{c}{P}\\ \hline
\multirow[c]{4}{*}{\rotatebox[origin=tr]{90}{{\footnotesize \textit{True}}}}
& N  &  3671 & 110 & 36 & 12         \\
& L   & 299 & 961 & 16 & 15      \\ 
& A  & 36 & 8 & 115 & 0        \\
& L   & 18 & 12 & 4 & 44       \\ \hline
% \bottomrule
\end{tabular}\hfil
\quad% ---------------------------
\begin{tabular}{cc|cc}
\centering
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{2}{c}{{\footnotesize \textit{Predicted}}} \\ 
\multicolumn{1}{c}{\textbf{\textcolor{CadetBlue}{AC}}} & 
\multicolumn{1}{c|}{} & 
\multicolumn{1}{c}{H} & 
\multicolumn{1}{c}{L} \\ \hline
\multirow[c]{3}{*}{\rotatebox[origin=tr]{90}{\textit{True}}}
& L  &  4954 & 99  \\[3ex]
& H   & 113 & 191 \\ \hline
\end{tabular}\hfil\hfil
\quad% ---------------------------
\begin{tabular}{cc|cc cc}
\centering
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{2}{c}{{\footnotesize \textit{Predicted}}} \\ 
\multicolumn{1}{c}{\textbf{\textcolor{CadetBlue}{PR}}} & 
\multicolumn{1}{c|}{} & 
\multicolumn{1}{c}{L} & 
\multicolumn{1}{c}{N} &
\multicolumn{1}{c}{H}\\ \hline
\multirow[c]{4}{*}{\rotatebox[origin=tr]{90}{\textit{True}}}
& L  &   2876 & 275 & 100       \\[1.3ex]
& N   & 404 & 1086 & 162     \\ [1.3ex]
& H   & 58 & 84 & 312      \\ \hline
\end{tabular}\hfil\hfil\vspace{3ex}
\quad% ---------------------------

% ==============================================dummy
\begin{tabular}{c p{1cm}}
 &   \\[1.5ex]
 &  \\ 
\end{tabular}\hfil\vspace{3ex}
\quad\quad% ---------------------------
% ==============================================dummy
\begin{tabular}{cc|cc}
\centering
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{2}{c}{{\footnotesize \textit{Predicted}}} \\ 
\multicolumn{1}{c}{\textbf{\textcolor{CadetBlue}{UI}}} & 
\multicolumn{1}{c|}{} & 
\multicolumn{1}{c}{R} & 
\multicolumn{1}{c}{N} \\ \hline
\multirow[c]{3}{*}{\rotatebox[origin=tr]{90}{\textit{True}}}
& R  &  3667 & 145  \\[3ex]
& N   & 229 & 1316 \\ \hline
\end{tabular}\hfil
\quad% ---------------------------
% ==============================================dummy
% \begin{tabular}{c p{1cm}}
%  &   \\[1.5ex]
%  &  \\ 
% \end{tabular}\hfil\vspace{3ex}
% \quad\quad% ---------------------------
% ==============================================dummy
\begin{tabular}{cc|cc}
\centering
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{2}{c}{{\footnotesize \textit{Predicted}}} \\ 
\multicolumn{1}{c}{\textbf{\textcolor{CadetBlue}{S}}} & 
\multicolumn{1}{c|}{} & 
\multicolumn{1}{c}{U} & 
\multicolumn{1}{c}{C} \\ \hline
\multirow[c]{3}{*}{\rotatebox[origin=tr]{90}{\textit{True}}}
& U  &  4323 & 133   \\[3ex]
& C   & 169 & 732  \\ \hline
\end{tabular}\hfil\vspace{3ex}
% ==============================================dummy
\begin{tabular}{c p{1cm}}
 &   \\[1.5ex]
 &  \\ 
\end{tabular}\hfil\vspace{3ex}
\quad% ---------------------------
% ==============================================dummy
\begin{tabular}{cc|cc cc}
\centering
\multicolumn{1}{c}{} &\multicolumn{1}{c}{}& \multicolumn{2}{c}{{\footnotesize \textit{Predicted}}} \\ 
\multicolumn{1}{c}{\textbf{\textcolor{CadetBlue}{C}}} & 
\multicolumn{1}{c|}{} & 
\multicolumn{1}{c}{L} & 
\multicolumn{1}{c}{N} &
\multicolumn{1}{c}{H}\\ \hline
\multirow[c]{3}{*}{\rotatebox[origin=tr]{90}{\textit{True}}}
& L  & 2759 & 139 & 201        \\
& N   & 198 & 797 & 55     \\ 
& H  & 259 & 46 & 903       \\ \hline
\end{tabular}\hfil
\quad% ---------------------------
\begin{tabular}{cc|cc cc }
\centering
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{2}{c}{{\footnotesize \textit{Predicted}}} \\ 
\multicolumn{1}{c}{\textbf{\textcolor{CadetBlue}{I}}} & 
\multicolumn{1}{c|}{} & 
\multicolumn{1}{c}{L} & 
\multicolumn{1}{c}{N} &
\multicolumn{1}{c}{H}\\ \hline
\multirow[c]{3}{*}{\rotatebox[origin=tr]{90}{\textit{True}}}
& L  &    2346 & 73 & 221        \\
& N   & 154 & 724 & 58     \\ 
& H   & 296 & 36 & 1449        \\ \hline
\end{tabular}\hfil
\quad% ---------------------------
\begin{tabular}{cc|cc cc}
\centering
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{2}{c}{{\footnotesize \textit{Predicted}}} \\ 
\multicolumn{1}{c}{\textbf{\textcolor{CadetBlue}{A}}} & 
\multicolumn{1}{c|}{} & 
\multicolumn{1}{c}{L} & 
\multicolumn{1}{c}{N} &
\multicolumn{1}{c}{H}\\ \hline
\multirow[c]{3}{*}{\rotatebox[origin=tr]{90}{\textit{True}}}
& L  &    2703 & 261 & 43        \\
& N   & 290 & 1909 & 12    \\ 
& H   & 56 & 32 & 51       \\ \hline
\end{tabular}\hfil
\par\bigskip
% -----------------------------------------------------
\label{tab:cvss_confmatrix}
\caption{Confusion matrix for the proposed model.\colorbox{yellow}{any idea to make table more organized?}}
\end{table}

\noindent \textbf{Shortages and Limitations--}\\
As mentioned earlier, CVEs typically fail provide all key information about the CVSS metrics. For example, Table \ref{tab: CVSS_misclass_example} shows the description of CVE-2012-1516 that is describing a vulnerability in VMware. The "Attack Complexity" metric describes "\textit{the conditions beyond the attacker's control that must exist in order to exploit the vulnerability. Such conditions may require the collection of more information about the target, the presence of certain system configuration settings, or computational exceptions}" \footnote{https://www.first.org/cvss/v3.0/specification-document}. This is a pretty deep and conceptual definition requiring some background knowledge and fine-grain information about the vulnerability to specify if this metric corresponding to the give, CVE is highly or lowly complex. 
Based on the vendor report, the only required condition for this attack is for virtual machines to have 4GB of memory and virtual machines with less than 4GB of memory are not affected, and hence,  the "Attack Complexity" is specified as "Low" for this CVE. 
The CVE description (see Table \ref{tab: CVSS_misclass_example}) clearly failed to provide such detailed information (i.e., the 4GB RAM need), making it pretty challenging even for  an expert to predict the metric value based on the provided text. 
\begin{table}[!ht]
\small
\centering
 \begin{tabular}{|l | l |} 
\hline 
 \multicolumn{2}{p{14cm}}{\textbf{CVE-2012-1516}: \textit{The VMX process in VMware ESXi 3.5 through 4.1 and ESX 3.5 through 4.1 does not properly handle RPC commands, which allows guest OS users to cause a denial of service (memory overwrite and process crash) or possibly execute arbitrary code on the host OS via vectors involving data pointers.}} \\
  \hline

   \multicolumn{1}{|l|}{\textbf{Attack Complexity}} & \multicolumn{1}{|p{10cm}|}{High} \\
   \hline
  \multicolumn{1}{|l|}{\textbf{Reason}} &
  \multicolumn{1}{|p{10cm}|}{The only required condition for this attack is for virtual machines to have 4GB of memory. Virtual machines that have less than 4GB of memory are not affected} \\
   \hline
\end{tabular}\hfil
     \caption{\label{tab: CVSS_misclass_example} Shows an example of uninformative CVE description for the purpose of "Attack Complexity" metric prediction.}
\end{table}

CVE database comprises many similar reports making both manual or automated CVSS perdition hard or even infeasible, solely based on the description.  Some works leveraged other standards such as CWEs to enrich the CVE texts for better prediction. However, this is highly problematic and leads to inconsistency since such standards represents the threats with a high level view and may not provide fine-grain information about the vulnerability's detailed behavior.  
The complementary solution to improve automated CVSS prediction is to use third-party resources such as vendor's vulnerability reports where in some cases, they provide low-level information about the vulnerabilities from different angles such as impacts, platforms, specific permissions, techniques, tactics, and procedures. In this case, a powerful text analytic tool such as SecureBERT can be utilized to process the context and analyze the semantic relationships, and possibly extract particular actions and features to represent each metric, if the information is provided within the input text. 

\section{Conclusions and Future Works}
In this work, we proposed a proof-of-concept framework that combines the SecureBERT cybersecurity domain-specific language model and a TF-IDF module to identify contextual information and extract key statistical features in order to predict the CVSS base vector for any given CVE based only on the text description. We conducted a rigorous and comparative evaluations and discussed the advantages and limitations of the model in details, and recommended potential solutions to make the automated CVSS prediction robust and effective.
Our approach performs well in detecting the values of particular metrics if the CVEs contain any important information about that metric, and outperforms all existing works in terms of individual metric prediction.

